MatchFormer: Interleaving Attention in Transformers for Feature Matching

Local feature matching is a computationally intensive task at the subpixel level. While detector-based methods coupled with feature descriptors struggle in low-texture scenes, CNN-based methods with a sequential extract-to-match pipeline, fail to make use of the matching capacity of the encoder and tend to overburden the decoder for matching. In contrast, we propose a novel hierarchical extract-and-match transformer, termed as MatchFormer. Inside each stage of the hierarchical encoder, we interleave self-attention for feature extraction and cross-attention for feature matching, yielding a human-intuitive extract-and-match scheme. Such a match-aware encoder releases the overloaded decoder and makes the model highly efficient. Further, combining self- and cross-attention on multi-scale features in a hierarchical architecture improves matching robustness, particularly in low-texture indoor scenes or with less outdoor training data. Thanks to such a strategy, MatchFormer is a multi-win solution in efficiency, robustness, and precision. Compared to the previous best method in indoor pose estimation, our lite MatchFormer has only 45% GFLOPs, yet achieves a +1.3% precision gain and a 41% running speed boost. The large MatchFormer reaches state-of-the-art on four different benchmarks, including indoor pose estimation (ScanNet), outdoor pose estimation (MegaDepth), homography estimation and image matching (HPatch), and visual localization (InLoc).

==> tables/outpose_more.tex <==
\resizebox{\columnwidth}{!}{
\renewcommand\arraystretch{1.5}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Method}}   &Data  &                                   \multicolumn{3}{c}{Pose estimation AUC} & \multicolumn{1}{c}{\multirow{2}{*}{P}} \\
    \cline{3-5}
                                                                     &   percent    & @5\degree & @10\degree & @20\degree           \\
    \midrule \midrule
    SP~\cite{detone2018superpoint}+SuperGlue~\cite{sarlin2020superglue} (1600)      &          & 42.18     & 61.16      & 75.95   & -- & --\\
    DRC-Net~\cite{li2020dual} (400) &  &27.01 &42.96 &58.31& --& --\\
    LoFTR-DS~\cite{sun2021loftr} (840) &  & {52.80} & {69.19}  & {81.18} & 94.8 & 600\\
    MatchFormer (640)    &           &  49.44     &  65.75       &  77.94  & 94.5  & 30 \\
    MatchFormer (840)  &         &49.83  &66.21   &78.92  &{95.1}  &350 \\
    \bottomrule
\end{tabular}
}
